Optimization-based Learning for Dynamic Load Planning in Trucking Service Networks

The load planning problem is a critical challenge in service network design for parcel carriers: it decides how many trailers to assign for dispatch over time between pairs of terminals. Another key challenge is to determine a flow plan, which specifies how parcel volumes are assigned to planned loads. This paper considers the Outbound Load Planning Problem (OLPP) that considers flow and load planning challenges jointly in order to adjust loads and flows as the demand forecast changes over time before the day of operations in a terminal. The paper aims at developing a decision-support tool to inform planners making these decisions at terminals across the network. The paper formulates the OLPP as a mixed-integer programming model and shows that it admits a large number of symmetries in a network where each commodity can be routed through primary and alternate terminals. As a result, an optimization solver may return fundamentally different solutions to closely related problems, confusing planners and reducing trust in optimization. To remedy this limitation, this paper proposes a lexicographical optimization approach that eliminates those symmetries by generating optimal solutions staying close to a reference plan. Moreover, this paper designs an optimization proxy that addresses the computational challenges of the optimization model. The optimization proxy combines a machine-learning model and a repair procedure to find near-optimal solutions that satisfy real-time constraints imposed by planners in the loop. An extensive computational study on industrial instances shows that the optimization proxy is orders of magnitude faster for generating solutions that are consistent with each other. The proposed approach also demonstrates the benefits of the OLPP for load consolidation and the significant savings obtained from combining machine learning and optimization.

==> 3stage_heuristic.tex <==
This heuristic leverages the idea that commodities, typically, adhere to their primary flow plans from a terminal, but, if there are better consolidation opportunities, then they might follow an alternate flow plan. First, the heuristic assigns the volume of each commodity to the sort pair defined by the primary flow plan; this step gives the final total commodity volume assigned to each sort pair. Then, we solve an integer program to decide the best combination of equipment types to be installed on the sort pairs as shown in model \ref{heuristic2}. This is the minimum knapsack problem which is known to be weakly NP-Hard, but can be solved efficiently using dynamic programming and can even be pre-computed for every sort pair.
\begin{subequations}\label{heuristic2}
    \begin{align}
    \underset{y}{\text{Minimize}} \ \quad &   \sum_{s \in S} \sum_{v \in V_s} c_{s,v} y_{s,v} \label{heur2_obj}\\
    \text{subject to} 
         \ \quad & \beta_s \leq \sum_{v \in V_s}Q^v (y_{s,v}), & \quad \forall  s \in S, \label{heur2_load}\\
         \ \quad & y_{s,v} \in \mathbb{Z}_{\geq 0} & \quad \forall s \in S, v \in V.  \label{heur2_nonneg}
    \end{align}
\end{subequations}

% In the third stage we fix the capacity, determined by the second stage, one each sort pair. Let $\widehat{S} \subseteq S$ be the set of sort pairs that are assigned non-zero capacity. For any sort pair $s \in S \backslash \widehat{S}$ we assign one unit of any equipment type $v \in V_s$; we can use planner's expert knowledge or historical data to determine such equipment types. Let the fixed units of equipment type $v$ on sort pair $s$ be denoted by $y^*_{s,v}$. Now we can solve a linear program as shown in \ref{heuristic3}.

% \begin{subequations}\label{heuristic3}
%     \begin{align}
%     \underset{x}{\text{Minimize}} \ \quad &   \sum_{k \in K}\sum_{s \in S_k}\sum_{v \in V_s}d^k_s x^k_{s,v} \label{heur3_obj}\\
%     \text{subject to} 
%         \ \quad &\sum_{s \in S^k} \sum_{v \in V_s} x^k_{s,v} = q^k, & \quad \forall  k \in K,  \label{heur3_flow} \\
%         \ \quad & \sum_{v \in V_s}\sum_{k \in K:s \in S^k} x^k_{s,v}\leq \sum_{v \in V_s}Q^v (y^*_{s,v}), & \quad \forall  s \in S, \label{heur3_load}\\
%         \ \quad & x^k_{s,v} \geq 0 & \quad \forall k \in K, s \in S^k, v \in V_s,  \label{heur3_nonneg}
%     \end{align}
% \end{subequations}
% The objective function in \eqref{heur3_obj} minimizes the total cost of deviating volume of commodity from primary to alternate sort pairs. These deviations define the overflow triggers used by planners to promote better consolidations which results in lower transportation cost.




==> consistent_lp_results.tex <==
\subsection{Generating Load Plans Consistent with the Base Plan}\label{variant}
In this section we will describe strategies (model variants) to recommend load plan modifications that do not deviate too much from the base plan, and hence, are ``\textit{operationally feasible}''. These variants are very useful from the implementation point-of-view because planners are more amenable to small changes from the base plan as the changes are easy to explain and implement. Intuitively, these model variants can be thought of as \textit{local search} techniques to generate the best load plan in a defined \textit{neighbourhood} of the base plan. Through empirical experiments we will show that even if we stick to the base plan with simple strategies, our plans are more effective, i.e., they have lower trailer cost and higher utilization.
% without drastic changes at the terminal in terms of trailer repositioning.
% Furthermore, these model variants give us more insight into the 

\subsubsection{Planned Trailer Units (PTU) Aware Model}
We introduce upper-bounds on the $y_{s,v}$ variables, defined in Model \ref{CreateLoadsModel}, to yield an MIP model which is aware of the total number of planned trailers units (\textit{PTU}) of a specific type $v \in V_s$ installed on each sort pair $s \in S$ in the base plan. The key idea here is to avoid using too many trailers on a particular sort pair and too few on other sort pairs; note that this is possible because the primary and alternate flow paths might allow assigning large commodity volume on some sort pairs (to achieve optimal consolidation) which necessitates installing many trailers on some of the sort pairs. As a result, some of the downstream nodes might have too many trailers and some might receive very few or no trailers.

To avoid generating such load plans, we add upper-bounds on $y$-variables as shown in \eqref{ub_on_y} such that we do not use more than the number of units of planned trailers, $\beta_{s,v}$, of type $v \in V_s$ on sort pair $s \in S$ in the base plan. As terminal planners build load plans based on their familiarity with the daily commodity volume at the terminal and outbound geographic destinations from the terminal, these upper-bounds help in developing plans that are easier for them evaluate. Intuitively, this proposed model variant take's a planner's base plan and tries to optimize consolidation and transportation cost. \textcolor{blue}{update the following inequality to load pair level.} 
\begin{align}
    y_{s,v} \leq \beta_{s,v}, & \quad \forall  s \in S, v \in V_s \quad \label{ub_on_y}
\end{align}
We refer to the resulting MIP model as Model \ref{CreateLoadsModel} with PTU and Table \ref{model1_ptu_stats} presents the computational statistics for the model. Note that the optimal objective function value of Model \ref{CreateLoadsModel} yields a lower-bound to the optimal objective function value of Model \ref{CreateLoadsModel} with PTU because every feasible solution of Model \ref{CreateLoadsModel} with PTU is a feasible solution of Model \ref{CreateLoadsModel}, but the converse is not true.

\begin{table}[!htbp]
\centering
\caption{Computational Statistics for Model \ref{CreateLoadsModel} with PTU} 
\begin{tabular}{l|r|r|r}
\toprule
Instance & FGap$\%$ & BGap$\%$ &  T(s) \\
\midrule
XS & 0.00 & 0.00 & 0  \\
S & 0.11 & 0.00 & 410\\
M1 & 0.08 & 0.00 & 1,679 \\
M2 & 0.00 & 0.00 & 5 \\
L1 & 3.85 & 1.88 & 1,800 \\
L2 & 2.58 & 1.17 & 1,800 \\
XL & 7.2 & 2.27 & 1,800\\
\bottomrule
\end{tabular}
\label{model1_ptu_stats}%
\end{table}%


% \subsubsection{Scheduled Sort Pairs}
% Based on historical commodity volume and planned loads,  planners consistently use a set of outbound sort pairs from each terminal; they might use different trailer type and units depending on the forecasted demand for a specific plan date. Note that the model \eqref{CreateLoadsModel} might prefer to use only a subset of the outbound sort pairs ($S$) in the optimal solution. For example, planners might operate $8$ trailers on $8$ (out of $10$) outbound sort pairs from a terminal, one on each sort pair, however, model \ref{CreateLoadsModel} might use the $8$ trailers on only $4$ out of the $10$ outbound sort pairs, $2$ trailers on each sort pair. The 

% \begin{align}
%     \sum_{v \in V_s}y_{s,v} \geq 1, & \quad \forall  s \in S^{sch} \label{op_feas}
% \end{align}

% \begin{table}[!htbp]
% \centering
% \caption{Computational Statistics for Model \ref{CreateLoadsModel} with Capacity Threshold and Scheduled Sort Pairs} \begin{tabular}{l|r|r|r}
% \toprule
% Instance & FGap$\%$ & BGap$\%$ &  T(s) \\
% \midrule
% XS & 0.00 & 0.00 & 0  \\
% S & 0.06 & 0.00 & 405\\
% M1 & 0.02 & 0.00 & 1379 \\
% M2 & 0.00 & 0.00 & 2 \\
% L1 & 3.32 & 2.88 & 1800 \\
% L2 & 1.90 & 1.42 & 1800 \\
% XL & 14.50 & 1.74 & 1800\\
% \bottomrule
% \end{tabular}
% \label{LargeT}%
% \end{table}%


\subsubsection{Optimizing for $\delta$-Volume}
In this section, we present a \textit{fix-and-optimize} framework where we \textit{fix} some commodity volume to be allocated to specific trailers on a sort pair, based on information from the base plan, and optimize for the remaining commodity volume. 

The first step in this process is to identify trailers that are planned to be at full capacity in the base plan. We develop a simulator which sorts the shipments processed at the terminal (recall that a set of shipments with the same destination and service class constitute a commodity) by arrival time, and packs them into the first available trailer (planned to be at full capacity) on the compatible (primary or alternate) sort pair in the base plan. Once the trailer is loaded to its full capacity, it is replaced by the second trailer planned to be at full capacity. The simulator stops when all the trailers, that were planned to be at full capacity, are loaded. The final step is to solve model \ref{CreateLoadsModel} for the residual commodity volume, which we refer to as $\delta-$Volume, and the remaining set of trailers across all the sort pairs. An illustration of this process is shown in Figure \ref{delta_example}.

\begin{figure}%[!htbp]
    \begin{subfigure}[t]{0.52\textwidth}
        \includegraphics[width=\textwidth]{figures/delta_1.pdf}
        \caption{Model \ref{CreateLoadsModel} would ignore the four planned trailers and independently plan loads for the eight shipments} \label{delta1}
     \end{subfigure}%
     \hfill
    \begin{subfigure}[t]{0.42\textwidth}
        \includegraphics[width=\textwidth]{figures/delta_2.pdf}
        \caption{Model \ref{CreateLoadsModel} with $\delta-$Volume would load and fix two trailers with six shipments, and solve Model \ref{CreateLoadsModel} for two shipments} \label{delta2}
     \end{subfigure}%
     \caption{Illustration to distinguish between Model \ref{CreateLoadsModel} and Model \ref{CreateLoadsModel} with  $\delta-$Volume. The example consists of three outbound destinations, eight shipments and four trailers, with two of them planned to be at full capacity indicated by stars.} \label{delta_example}
\end{figure}

\begin{table}%[!htbp]
\centering
\caption{Computational Statistics for Model \ref{CreateLoadsModel} with $\delta$-Capacity and $\delta$-Volume} \begin{tabular}{l|rrrrrrrr}
\toprule
Instance & Fixed Volume & $\delta$-Volume &\#Int-Vars & \#Cont-Vars & \#Cons & FGap$\%$ & BGap$\%$ &  T(s) \\
\midrule
XS & $50\%$ & $50\%$ & 16 & 3,270 & 1,310 & 0& 0 & 0\\
S & $50\%$ & $50\%$& 72 & 9,716 & 2,889 & 0.07 & 0.04 & 1800\\
M1 & $64\%$ & $36\%$& 187 & 19,613 & 2,979 & 0.02 & 0.01 & 1800\\
M2 & $38\%$ & $62\%$& 220 & 19,393 & 6,375 & 0 & 0 & 4\\
L1 & $69\%$ & $31\%$& 859 & 29,393 & 6,662 & 2.87 & 2.49 & 1800\\
L2 & $66\%$ & $34\%$& 846 & 32,059 & 8,495 & 2.38 & 2.07 & 1800\\
XL & $67\%$ & $33\%$& 4,745 & 57,173 & 15,154 & 4.53 & 2.98 & 1800\\
\bottomrule
\end{tabular}
\label{model1_delta_vol}%
\end{table}%

In table \ref{model1_delta_vol}, column \textit{Fixed Volume} denotes the percentage of total commodity volume ($\sum_{k \in K}q^k$) allocated to trailers on  a compatible sort pair and column \textit{$\delta$-Volume} denotes the percentage of total commodity volume for which Model \ref{CreateLoadsModel} is solved. In this model variant were able to fix around $50\%-60\%$ of commodity volume and optimize for the remaining $40\%-50\%$. Table \ref{model1_delta_vol} shows that the number of integer variables remains the same but there are fewer continuous variables and constraints in Model \ref{CreateLoadsModel} with $\delta-$Volume as compared to Model \ref{CreateLoadsModel}. Recall that the $x$-variables and constraints \eqref{FlowAssignment} in Model \ref{CreateLoadsModel} depend on the set of commodities which is smaller in Model \ref{CreateLoadsModel} with $\delta-$Volume due to fixed trailer allocation for some shipments (and hence, commodities). The computational statistics in Table \ref{model1_delta_vol} show that all the instances can be solved to reasonable optimality gap for implementation in real-life operations for our industry partner.


\begin{figure}[!htbp]
    \begin{subfigure}[t]{0.48\textwidth}
        \includegraphics[width=\textwidth]{figures/XS.pdf}
        \caption{XS} \label{XS}
     \end{subfigure}%
     \hfill
    % \hspace*{0.2\textwidth}   % maximize separation between the subfigures
    \begin{subfigure}[t]{0.48\textwidth}
        \includegraphics[width=\textwidth]{figures/S.pdf}
        \caption{S} \label{S}
     \end{subfigure}%
     \hfill
    \begin{subfigure}[t]{0.48\textwidth}
        \includegraphics[width=\textwidth]{figures/M1.pdf}
        \caption{M1} \label{M1}
     \end{subfigure}%
     \hfill
    \begin{subfigure}[t]{0.48\textwidth}
        \includegraphics[width=\textwidth]{figures/M2.pdf}
        \caption{M2} \label{M2}
     \end{subfigure}%
     \hfill
    \begin{subfigure}[t]{0.48\textwidth}
        \includegraphics[width=\textwidth]{figures/L1.pdf}
        \caption{L1} \label{L1}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{0.48\textwidth}
        \includegraphics[width=\textwidth]{figures/L2.pdf}
        \caption{L2} \label{L2}
    \end{subfigure}%
\end{figure}
\begin{figure}\ContinuedFloat
\captionsetup{subrefformat=\thefigure.(\alph{subfigure})}
    \begin{subfigure}[t]{0.48\textwidth}
        \includegraphics[width=\textwidth]{figures/XL.pdf}
        \caption{XL} \label{XL}
    \end{subfigure}%
    \caption{Operational Performance of the Modified Load Plans with respect to the Base Plan} \label{base_create_add_delta}
\end{figure}

Figures \ref{base_create_add_delta} demonstrates the performance of the Model \ref{CreateLoadsModel} and its variants relative to the base plan. We consider two metrics: \textit{$\%$ Utilization} and \textit{$\%$ diversion}, as calculated in \eqref{util} and \eqref{divert}
\begin{align}
    \% Utilization ={}& \frac{\text{total commodity volume}}{\text{total trailer capacity}} \label{util} \\
    \% Diversion ={}& \frac{\text{total commodity volume assigned to alternate flow paths}}{\text{total commodity volume}} \label{divert}
\end{align}
One clear observation is that higher trailer utilization is driven by higher diversion of commodity volume from primary flow paths to the alternate flow paths; Model \ref{CreateLoadsModel} and its variants achieve better objective function value, and hence, better consolidation by allocating some volume to the alternate flow paths. We observe that Model \ref{CreateLoadsModel} has the highest $\%$ Utilization and $\%$ diversion because it has the flexibility to install any number of trailers of a (compatible) type on each sort pair and achieves highest consolidation. Model \ref{CreateLoadsModel} with PTU has a restriction that it cannot use more trailers of a specific type on a given sort pair than there are in the base plan. Hence, it has lower $\%$ Utilization than Model \ref{CreateLoadsModel}, but, interestingly, it has better $\%$ Utilization than the \textit{Base Plan}. The reason is that Model \ref{CreateLoadsModel} with PTU is able to achieve better consolidation by allocating some volume to alternate flow paths than the \textit{Base Plan}. Model \ref{CreateLoadsModel} with $\delta-$Volume has the lowest $\%$ Utilization among the three model variants for all instances. Even then, it performs better than the \textit{Base Plan} for all instances except \textit{M2}. For the \textit{M2} instance, there are very few commodities (and the total volume is small due to \textit{fixing}) that can be allocated to alternate flow paths. Observe that $\%$ diversion is very small due to which the improvement in $\%$ Utilization is negligible for the \textit{Base Plan} and all model variants for instance \textit{M2}. 


==> greedy_heuristic.tex <==
\subsection{Iterative Greedy Heuristic}
Main idea: Mimic action of planners
\begin{itemize}
    \item Solver-free Heuristic
    \item \textit{Step 1: }Pick the best sort pair to install one unit of an equipment type. The term ``best'' refers to the sort pair that has enough volume (either from primary or alternate flow plans) to fill $100\%$ of the trailer.
    \item \textit{Step 2: }Assign volume to the trailer and update remaining volume on all the sort pairs. Go to \textit{Step 1}. 
\end{itemize}

\textcolor{blue}{Add details and examples}

==> iid_heuristic.tex <==
\subsection{Iteratively Discovering Integer Variables}



==> local_search.tex <==
Solve the linear program and round the solution to get a feasible solution.
\begin{enumerate}
    \item Check if removing an equipment on any sort pair yields a solution with a better objective value, if not, got to Step 2. If yes, then make the change and re-solve the linear program
    \item Check if removing an equipment on any sort pair and adding an equipment on another sort pair yields a solution with a better objective value, if not, stop.
\end{enumerate}

These heuristics exploit the idea that fixing the capacity on every sort pair results in a linear program which can be solved efficiently.

==> temp.tex <==
\section{Solution Approach}\label{solution}
\subsection{Exact Approaches}
Solving the MIP directly using a commercial solver.

\subsection{Greedy Iterative Variable Bounding}\label{GIVB}
In this section we present a heuristic algorithm that iteratively solves linear programs to construct a feasible solution to the outbound load plan modification problem. The heuristic is based on an idea that is often used by planners to determine trailer decisions.

Pseudocode \\

\begin{proposition}
GIVB is a pseudo-polynomial time algorithm
\end{proposition}
\begin{proof}
\textit{GIVB} solves a linear program in every iteration which can be solved in polynomial time. Now we will show that the number of iterations required to terminate the algorithm is polynomial in the size of the input. Observe that the heuristic updates the lower bound of one general integer variable in each iteration. At the start of each iteration the lower bound of each trailer variable $y_{s,v}$ is $lb(s,v) =0$. The integer upper bound of each variable $y_{s,v}$ can be calculated as $ub(s,v) = \left \lceil{\frac{\sum_{k \in : s \in S^k}q^k}{Q^v}}\right \rceil$. Note that in each iteration the $lb(s,v)$ will increase by at least one for some $(s,v)$ and it can increase to at most $ub(s,v)$; at this point the variable is fixed in the model, i.e., $y_{s,v} = ub(s,v)$. Therefore, the maximum number of iterations required to construct a feasible solution is $\sum_{s \in S}\sum_{v \in V_s}(ub(s,v)-lb(s,v))$ which depends on the size of the input data.

\end{proof}
% \section{Local Search Heuristic Algorithm}
% In this section we describe two-stage heuristic algorithms for solving Model \ref{CreateLoadsModel} where stage $1$ constructs a feasible solution and stage $2$ improves the feasible solution to get a local optimal solution.

% \subsection{Construction Phase}
% \textbf{Greedy Iterative Variable Bounding heuristic}: 
% % \input{givb_heuristic.tex}

% \textbf{Primary Load Plan Heuristic}: This heuristic leverages the idea that commodities, typically, adhere to their primary flow plans from a terminal, but, if there are better consolidation opportunities, then they might follow an alternate flow plan. First, the heuristic assigns the volume of each commodity to the sort pair defined by the primary flow plan; this step gives the final total commodity volume assigned to each sort pair. Then, we solve an integer program to decide the best combination of equipment types to be installed on the sort pairs as shown in model \ref{heuristic2}. This is the minimum knapsack problem which is known to be weakly NP-Hard, but can be solved efficiently using dynamic programming and can even be pre-computed for every sort pair.
% \begin{subequations}\label{heuristic2}
%     \begin{align}
%     \underset{y}{\text{Minimize}} \ \quad &   \sum_{s \in S} \sum_{v \in V_s} c_{s,v} y_{s,v} \label{heur2_obj}\\
%     \text{subject to} 
%          \ \quad & \beta_s \leq \sum_{v \in V_s}Q^v (y_{s,v}), & \quad \forall  s \in S, \label{heur2_load}\\
%          \ \quad & y_{s,v} \in \mathbb{Z}_{\geq 0} & \quad \forall s \in S, v \in V.  \label{heur2_nonneg}
%     \end{align}
% \end{subequations}

% \textbf{Iteratively Discovering Integer Variables}: Start with a linear programming relaxation at the root node (possibly with cutting planes identified at the root node). Iteratively identify new trailer decision variables that can be re-defined as integer or binary variables.

% \subsection{Improvememt Phase}
% Local Search

% \input{local_search.tex}

